Star Formation in the Milky Way and Nearby Galaxies

We review progress over the past decade in observations of large-scale star formation, with a focus on the interface between extragalactic and Galactic studies. Methods of measuring gas contents and star formation rates are discussed, and updated prescriptions for calculating star formation rates are provided. We review relations between star formation and gas on scales ranging from entire galaxies to individual molecular clouds.

==> exgal.tex <==
%milkyway.tex
% changed name to exgal.tex 080911 NJE
%updated 042611 NJE
% 061011 NJE
%070511 NJE
%070811 NJE
%070911 NJE
%080711 RCK (and many before)
%080911 NJE changed file name to exgal.tex and have it call milkyway.tex
% because I had edited milkyway.tex as a subsection. This is full section now.

\input milkyway.tex

\subsection{Demographics of Star-Forming Galaxies Today}\label{demographics}

The influx of new multi-wavelength data over the past decade not
only has expanded the richness of information available on global
star formation properties of galaxies; it also has transformed the
interpretive framework of these observations from only largely based
on characterising the Hubble morphological sequence to one based on
a quantitative foundation of galaxy luminosity, masses, and other
physical properties.  

The recognition of galaxy mass as a fundamental determinant of 
the star formation history of a galaxy predates the modern mega-surveys
(e.g., Gavazzi et al. 1996), but data from SDSS and subsequent large-area
surveys have estabished the bimodal dependence of SFR and
other properties on mass as the most common basis for interpreting
the Hubble sequence (i.e., Kauffmann et al. 2003; Baldry et al. 
2004, 2006; Brinchmann et al. 2004).  The integrated colors of galaxies,
which are sensitive to their star formation histories, show a strongly
bimodal dependence on stellar mass, with a relatively tight ``red
sequence" populated by galaxies with little or no star formation today,
and a somewhat broader ``blue sequence" or ``blue cloud" of actively
star-forming galaxies.  These sequences show separation both in color
and in galaxy mass.  In terms of color the relative dearth of galaxies 
in the ``green valley"
between the red and blue sequences suggests either a deeper underlying
physical bimodality in the galaxy population or a rapid evolution of
galaxies from blue to red sequences.  The proportions of galaxies
in the red and blue sequences transforms sharply around a stellar mass
of $\sim 3 \times 10^{10}$\,\msun\ (Kauffmann et al. 2003).

Some of the trends in the bimodal color-magnitude diagram for galaxies
simply mirror the well-established trends between star formation history
and galaxy type.  For example the color bimodality is driven in large
part by the morphological segregation of galaxies into spheroidal and
disk systems, and by the strongly suppressed star formation in bulge-dominated
disk galaxies (Kennicutt et al. 1994).  Nevertheless the new data offer
important new insights, not the least the strong mass dependence of the
galaxy populations and the relatively homogeneous properties of galaxies
within the red and blue sequences.

Within the context of this review the most interesting relation of
this type is the dependence on galaxy mass of the SFR per unit galaxy
mass, or the ``specific SFR" (sometimes abbreviated as SSFR).  This
parameter scales directly (via a factor of the age of galaxies) with
the stellar birthrate parameter $b$, the ratio of the SFR today to 
the average past SFR over the age of the galaxy.  These provide convenient
parametrizations of the mass-normalized or time-normalized SFRs today.
The mass dependence of the SSFR has been explored by numerous investigators
(e.g., Brinchmann et al. 2004; Salim et al. 2007; Schiminovich et al. 2007;
Bothwell et al. 2009), and Figure 5.1 shows an example from Schiminovich et al.
(2007), based in this case on dust-corrected FUV measurements of SDSS galaxies.  

[Figure 5.1 here]

This relation shows several characteristic features which are confirmed
in other studies.  As highlighted earlier the dispersion of SSFRs within
the blue sequence is suprisingly tight, suggesting some self-regulation
mechanism at work among the actively star-forming galaxies.  There is
a clear tail of less active but significantly star forming galaxies
above the red sequence;
as described below these are a combination of relatively inactive disk
galaxies and unusually active spheroid-dominated systems.  The sharp
increase in the fraction of red galaxies above stellar masses of order
a few times 10$^{10}$\,\msun\ is also seen.   Also clearly seen in these
data is a systematic increase in SSFR with decreasing galaxy mass on the
blue sequence.  The slope measured for this tilt varies somewhat between
different studies, possibly reflecting the effects of different sampling
and incompletness biases in the respective surveys; in Figure 5.1 the
power-law slope is $-0.36$.  This implies that lower-mass galaxies are
forming a relatively higher fraction of their stellar mass today, and
conversely must have formed stars less efficiently relatively to their
massive galaxy counterparts at earlier cosmic epochs.

As a result of this dependence star formation in the Universe today
is weighted to considerably lower galaxy masses than the respective
weighting of stellar mass itself.  A simple way to explain this trend
would be to hypothesise that over recent cosmic time star formation
has gradually migrated from more massive to less massive galaxies.
Indeed direct evidence for this ``downsizing" is seen in observations
of the SFFR vs mass relation in high-redshift galaxies  
e.g., Noeske et al. 2007).

Another illuminating way to parametrize the properties of the star-forming
population is solely in terms of the SFRs themselves, either
in absolute terms or normalised per unit galaxy mass (SSFR) or
per unit area (SFR density or intensity).  Figure 5.2 shows the
distribution of SFRs per unit area plotted as functions of the
absolute SFRs from a compilation of data from several surveys.
Normal disk and irregular galaxies, plotted as solid points are
from a volume-complete H$\alpha$ survey of the local 11 Mpc volume
by Kennicutt et al. (2006), the diameter-limited H$\alpha$GS survey
of James et al. (2004), and the GOLDMINE survey of the Virgo cluster
by Gavazzi et al. (2003, and references therein).  All \halpha\
luminosities were corrected statistically for dust attenuation,
and galaxy radii correspond to those of the active star-forming
disks, as measured from the \halpha\ images.  Red points denote
luminous infrared galaxies (LIRGs) and ultraluminous infrared galaxies
(ULIRGs) from the surveys of Dopita et al. (2002) and the compilation
of Scoville et al. (1999), but with AGN-dominated galaxies removed.
The SFRs of these galaxies were measured from their TIR luminosities,
though in a few cases when possible from dust-corrected \halpha\ fluxes.
Blue points are blue compact starburst galaxies from the \halpha\ surveys
of Gil de Paz (2003) and Perez-Gonzalez et al. (2003), again with 
SFRs corrected for dust attenuation.  The green points denote
circumnuclear starbursts, mostly measured in Pa$\alpha$, from the
compilation in Kormendy \& Kennicutt (2004).   Finally the violet
point roughly denotes the position of the Milky Way, based on the
SFRs described in the previous section.  No effort has made
to compile complete or fully respresentative subsamples of these
galaxies (indeed the LIRGs and ULIRGs were drawn from space volumes
that are thousands of times larger than the other galaxies, and hence
are grossly over-represented in absolute numbers).  Instead we
compile the diagram to illustrate the orders-of-magnitude diversity
in star formation properties in the local Universe.

[Figure 5.2 here]

Several interesting conclusions can be drawn from the data in Figure 5.2.
The first is the extraordinary range in SFRs, more than 7 orders of
magnitude, whether measured in absolute terms or normalized per unit
area or (not shown) galaxy mass.  Much of this range is contributed however
by non-equilibrium systems, various classes of starbursts.  The
normal galaxies occupy a relatively tight range of SFRs per unit area,
reminiscent of the tightness of the blue sequence when expressed in
terms of SSFRs.  The total SFRs of the quiescent star-forming galaxies
are also tightly bounded below a value of $\sim$20\,\msun\,yr$^{-1}$.
Starburst galaxies, and infrared-luminous and ultraluminous systems
in particular, comprise most of the galaxies in the upper 2--3 decades
of absolute SFRs and SFRs per unit area.

The distribution of SFRs along the X-axis of Figure 5.2 (making
proper accounting for volume-complete statistics) is simply the
SFR distribution function.  This function has been measured by a
number of workers beginning with Gallego et al. (1995), and a recent
determination based on GALEX and IRAS catalogs and the Local Volume
Legacy Survey (Dale et al. 2010; Lee et al. 2011) was published recently
by Bothwell et al. (2011).  Figure 5.3 shows the resulting SFR distribution
function, derived from a combination of FUV and TIR fluxes as calibrated
by Hao et al. (2011).  An important ingredient in such analyses is the removal of
the AGN contribution to heating in the TIR dust luminosities.  Several
years ago this was problematic but the advent of mid-IR spectroscopy
has made it possible to apply individual or statistical corrections 
for the AGN contributions (Wu et al. 2011 and references therein).
The SFR function is well fitted by a Schechter (1976) exponentially
truncated power-law, with a faint-end slope $\alpha = -1.5$ and 
SFR$^*$ = 9\,\msun.  The fact that the this value remains low despite
the presence of LIRGs and ULIRGs in the local Universe testifies to the
very small contribution ($<10$\%\, also see Goto et al. 2010).
Star formation at $z=0$ is overwhelmingly dominated by quiescent normal
star-forming disk galaxies.  
The situation is quite different at high-redshift, where SFR$^*$
increases rapidly and galaxies with bolometric luminosities of 
more than 10$^{11}$\,L$_\odot$ become dominant by redshifts $z > 1$
(e.g., Le Floc'h et al. 2005).


[Figure 5.3 here]

An important byproduct of these multi-wavelength surveys has been
the quantifying of a strong systematic correlation between the mean
dust attenuation in the UV and visible and the total SFR of the galaxy
(e.g., Wang \& Heckman 1996; Martin et al. 2005).  This correlation
is probably a second-order consequence of the Schmidt law, with the
most intense star formation taking place in regions of the highest
gas-- and thus also dust-- surface densities.  As a consequence 
the high-SFR tail ($>$SFR$^*$) of the present-day distribution is
dominated by heavily dust-obscurred galaxies, mostly LIRGs and
ULIRGs.

\subsection{Star Formation in the High-Density Regime: Starbursts}
\label{starbursts}

As reviewed in K98 the starburst phenomenon encompasses a wide
range of physical scales and host galaxy properties.  Although
a universally adopted definition does not exist, the term commonly
is applied to galaxies with SFRs which cannot be sustained for
longer than a small fraction (e.g., $\le$10\%) of the Hubble time,
i.e., with gas consumption timescales of less than $\ge$100 Myr.
As the wavelength range of extragalactic observations has expanded
new classes of starburst galaxies have been discovered and categorised,
for example LIRGs and ULIRGs in the infrared, blue compact galaxies
(BCGs), blue compact dwarfs (BCD's), HII galaxies, clumpy irregular 
galaxies, and Wolf-Rayet galaxies in the visible, Lyman-alpha and
UV-luminous galaxies in the ultraviolet, and Lyman-break, BzK,
and submillimeter galaxies at high redshift.  Most of these classes
of galaxies are physically distinct but they all fit the general
definition of a starburst galaxy given above.  Moreover, as
Figure 5.2 demonstrates, many of these subjectively defined classes
of starburst galaxies are distinct from their more quiescent
counterparts; for example most starbursts possess SFR surface densities
above 0.1\,\msun\,yr$^{-1}$\,kpc$^{-2}$, much higher than is typical
for normal galaxies.  Roughly the same SFR density appears to 
mark the onset of large-scale outflows from the disks of star-forming
galaxies [reference needed].  Likewise, essentially by definition,
starbursts occupy a distinct locus in terms of SSFRs with a 
dividing line at a few times $10^{-10}$\,yr$^{-1}$ (i.e., 
birthrate parameter $b \gg 1$.  As discussed earlier starburst
galaxies also dominate the population of absolute SFRs above
$\sim$10\,\msun\,yr$^{-1}$, but many starburst galaxies have
much lower absolute SFRs, and the upper envelope in SFRs for
the main galaxy population increases rapidly with increasing redshift.

Although Figure 5.2 demonstrates that it is possible to
define quantitative criteria for starburst galaxies, either
in terms of SFR densities, absolute SFRs, or SSFRs, the data
also clearly show that there is no natural clean dichotomy
between normal star-forming galaxies and starbursts.  Instead
there is a continuum of SFRs, with starbursts defining the 
upper tails of the distributions in SFRs.

Much of the attention in this area continues to focus on the
infrared-luminous and ultraluminous systems, because they probe
star formation in the most extreme high-density circumnuclear
environments seen in the local Universe.  Until about a decade
ago studies of the most luminous systems was handicapped by
the difficulty in separating the component of dust emission
produced by young stars from the component heated by an active
galactic nucleus or AGN (Sanders \& Mirabel 1996).  Thanks to
new mid-infrared spectroscopic observations of these galaxies
with the ISO and Spitzer observatories this problem now is
largely solved.  Regions heated by AGNs show the characteristic
high-ionization signatures in their mid-infrared spectra, and
infrared analogs to the well-known optical forbidden-line diagnostic
diagrams (e.g., Baldwin et al. 1981) can be used to separate
the heating sources (e.g., Genzel et al. 1998, Dale et al. 2006, 
Armus et al. 2007).  Regions heated by AGNs also strongly 
suppressed mid-infrared PAH emission when compared to stellar
photoionized regions, and this can be used either separately
or in conjunction with gas ionization diagnostics to separate
the two and even estimate the relative fractions of dust
heated by stars and AGNs (e.g., Genzel et al. 1998, Wu et al.
2011).  This has made it possible to construct clean samples
of LIRGs and ULIRGs which are dominated by star formation,
and to separate the contributions of AGNs and starbursts to
the infrared luminosity function and SFR distribution function.

[Do we want to say anything about the Galactic center here?]

With the Spitzer and Herschel observatories it has been possible
to extend imaging and spectroscopy of the most luminous infrared-emitting
galaxies to intermediate redshifts (e.g., Elbaz et al. 2005, Yan et al. 2007).
As mentioned earlier the fraction of star formation in LIRGs and ULIRGs increases
sharply with redshift, but imaging and spectroscopy of these objects
reveals a marked shift in the physical characteristics of the population.
Whereas at low redshift ULIRGs (and many LIRGs) are dominated by 
very compact circumnuclear starbursts triggered by mergers, at
higher redshifts the LIRG/ULIRG population becomes increasingly
dominated by large disk galaxies with extended star formation.
These apparently are the high-SFR tail of the normal star-forming galaxy
population.  As a consequence of cosmic downsizing (i.e., ``upsizing" with increasing
redshift), normal massive galaxies by redshifts z$\sim$1 have SFRs
of tens of solar masses per year, and infrared luminosities well in
the regime of LIRGs or even ULIRGs.  These changes in population
are reflected in the spectra of the luminous galaxies, with strong
SFR signatures even at high luminosities which are dominated by AGNs
in the local Universe (Sanders \& Mirabel 1996).  Indeed composite
signatures of star formation as well as AGNs are often observed.
It is possible that distant analogs to the local population of
compact merger-driven ULIRGs are also present at high redshift,
especially in the submillimeter galaxy population, but the 
contribution of the ``main sequence" of extended star-forming
galaxies becomes increasingly important.  

Visible-wavelength observations of these high-redshift galaxies
with IFU instruments, both with and without adaptive optics correction,
have revealed many insights into the physical nature of this population
of starburst galaxies (e.g., Genzel et al. 2008, 2011; 
Forster-Schreiber et al. 2009 and references therein).  The 
H$\alpha$ kinematics show a wide range of properties from normal
differentially rotating disks to disturbed disks and a subset
with signatures of ongoing or recent mergers.  The disks tend
to be characterized by unusually high velocity dispersions, which
have been interpreted as reflecting a combination of dynamical
instability and possibly energy injection into the ISM from young
stars.  Further discussion of high-redshift galaxies is beyond
the scope of this article, but we shall return to the cold ISM
properties and SFRs of these galaxies in \S5.5.

\subsection{The Low Density Regime: Early-Type Galaxies, Extended
Disks, and Dwarf Galaxies}\label{earlytype}

One of the most important discoveries to come out of the GALEX
ultraviolet mission was the detection of low levels of star formation
in galaxies (and regions of galaxies) which often were thought to
have been devoid of star formation previously.  This new sensitivity
to extremely low levels of star formation derived from the combination
of the sensitivity of UV imaging to star formation (owing in turn to
a combination of the broad bandwidth and extended lifetimes of the
UV-emitting stars relative to H$\alpha$) and the exceptionally dark
UV sky background in space.  As a result GALEX observations, combined
with follow-up observations at other wavelengths, have revolutionised
our knowledge of star formation in early-type galaxies,
dwarf galaxies, low surface brightness galaxies, and the extreme
outer disks of many normal galaxies.

One of the most important of these contributions has been the
discovery of ongoing star-formation in a considerable fraction
of nearby early-type (E and S0) galaxies.  Prior to GALEX resolved
star formation had been detected in a few nearby elliptical and
S0 galaxies and peculiar objects such as NGC\,5128 = Cen A, but
the common interpretation of this component of the galaxy population
was well summarized by the phrase ``red and dead" which was often
applied to the red sequence in the SDSS color-magnitude plane.
Most of the UV emission that was detected in these galaxies was
thought to arise from evolved (e.g., post-AGB) stars.  However
GALEX imaging of SDSS galaxies has revealed approximately 30\%\
of early-type galaxies exhibit near-ultraviolet emission in
excess of what could reasonably arise from an evolved stellar
population (Yi et al. 2005, Kaveraj et al. 2007).  Interestingly
the optical colors of these galaxies place nearly all of them
tightly on the red sequence, which demonstrates the sensitivity
and need for UV observations to separate the young stellar component.
The SFRs tend to be very low, with at most 1--3\%\ of the stars
in the galaxies being formed over the past Gyr, if stars have
formed for that long at the present rates.  Visible-wavelength
IFU spectroscopy, as exploited for example by the SAURON survey,
has proven to be another powerful probe of low-level
star formation in early-type galaxies (e.g., Shapiro et al. 2010),
through both emission-line and stellar absorption line diagnostics.
Low-level star formation is common in disks of S0 galaxies
(e.g., Thilker et al. 2010),
and often found in more compact circumnuclear structures.
Follow-up CO observations of these galaxies reveals significant
detections of molecular gas in a large fraction of the galaxies
with detected star formation, 
with molecular gas masses of $10^7 - 10^{10}$\,\msun\
(Combes et al. 2007, Crocker et al. 2011), and with SFRs
roughly with the Schmidt law seen in normal galaxies.

The GALEX images also revealed that star formation in more
active disk galaxies is often far more extended in radius
that had previously been appreciated.  In exceptional cases
(e.g., NGC\,5236=M83, NGC\,4625) the star formation extends
to 3--4 times the normal $R_{25}$ optical radius, essentially
to the edge of the HI disk (Thilker et al. 2005, Gil de Paz 
et al. 2005).  These extended structures are now often referred
to as ``XUV" disks.  A systematic study of a larger sample 
of nearby galaxies reveals that $\sim$20\%\ of spiral galaxies
have star formation extending well beyond the main optical
disk, with distinct outer structues occurring in another 
10\% of galaxies.  The existence of star formation at large
radii is not a new observation; studies of HII regions at
large radii extend back to Munch (1959), Hodge (1969), 
and particularly Ferguson et al. (1998).  As with the 
study of star formation in early-type galaxies, the GALEX
observations have demonstrated the prevalence of star formation
at very large radii, and made it possible to conduct
detailed studies of the properties of the star-forming
regions in these low-density environments.  Early suggestions
that the extended disks only appeared in the ultraviolet and
not at H$\alpha$ have led to suggestions that the mode of
star formation or the IMF in these regions may be systematically
different from those in the inner disks (e.g., Pflamm-Altenburg
\& Kroupa 2008).  Subsequent combined UV and H$\alpha$
imaging and spectroscopy of the XUV disks (e.g., Zaritsky \&
Christlein 2007, Christlein et al. 2010, Goddard et al. 2010)
reveal however that when careful measurements of the H$\alpha$
emission are made taken proper account of sky background 
the profiles closely follow those observed in the ultraviolet
in most galaxies, and therefore strongly limit any systematic
difference in the IMF in those regions.  These preliminary
studies however have only begun to tap the potential of the
GALEX observations for probing the star formation and chemical
evolution properties of galaxy disks at very large radii.

The GALEX images also have led to a breakthrough in measurements
of star formation in low surface brightness spiral galaxies (LSBs).
These galaxies, for which the prototype is Malin 1 (Impey \&
Bothun 1989).  These galaxies are characterized by low bulge/disk
ratios, very extended disks, and disk surface brightnesses that
can be 10--100 times fainter than the characteristic values in
normal spiral galaxies.  Until recently most information on SFRs
in these systems were limited to a few unpublished H$\alpha$
observations, but GALEX has provided a homogeneous body of deep
measurements of the star formation in these systems (Wyder
et al. (2009).  These have been used to probe the low-density
extention to the star formation law, as discussed in the next section.

The other class of star-forming galaxies with unusually low
surface densities are the low surface brightness dwarf irregular
galaxies.  Historically any effort to draw general inferences 
about the star formation properties of these galaxies was limited
by the heterogeneity of the available datasets and selection biases
in the samples.  Over the past few years a number of groups have
attempted to address this problem by carrying out surveys
studies of well-defined volume-limited samples of nearby dwarf
galaxies (e.g., Blanton et al. 2005, Karachentsev et al. 2005,
Meurer et al. 2005, Kennicutt et al. 2008, Dalcanton et al. 2009).  When combined 
with large bodies of multi-wavelength observations of dwarf
galaxies (e.g., Hunter et al. 2010) a relatively complete
characterization of the star formation properties and histories
of low-mass gas-rich galaxies is beginning to emerge.

The most interesting results to emerge from these studies
are on the statistics of SFRs in the galaxies, which come mainly
from large surveys in H$\alpha$ and the far-ultraviolet, and 
on the temporal properties and integrated strengths of the 
star formation bursts in these systems, which come from a 
combination of statistics in H$\alpha$ and the UV and time-resolved
studies based on deep color-magnitude diagrams.  Perhaps the
most striking result of all is the ubiquity of star formation
in the dwarf galaxies.  Kennicutt et al. (2008) observed or 
compiled H$\alpha$ luminosities for galaxies within the local
11 Mpc, which included $\sim$300 dwarf galaxies (M$_B > -17$).
Excluding a handful of dwarf spheroidal galaxies which have
no cold gas, only 10 of these ($\sim$3\%) were not detected in H$\alpha$,
indicating an absense of massive star formation in the last 3--5 Myr.
Follow-up imaging with GALEX (Lee et al. 2011) reveals 
clumped UV emission in some of these (not all of the H$\alpha$
nondetections have deep UV imaging), indicative of str formation over the
past 100--200 Myr.  Very recent star formation was observed in
all of the galaxies with M$_B < -13$ and 
$M(HI) > 5 \times 10^7$\,\msun.  For less massive galaxies
it is possible for star formation to cease for timescales that
are longer than the ionization lifetime of an HII region
(up to 5 Myr), but examples of galaxies with extended periods
of no star formation are extremely rare.  As pointed out by
Lee et al. (2011) the extreme dwarf regime (M$_B > -13$ and 
$M(HI) < 5 \times 10^7$\,\msun) is relatively unexplored, and
it would be interesting to test where this apparent ubiquity
of quasi-continuous star formation breaks down.

These data allow for a fresh look at the temporal properties
of the star formation in dwarf galaxies generally.  The
distribution of SSFRs shows a marked increase
in dispersion for galaxies with M$_B > -14.5$ or circular
velocity of 50\,km\,s$^{-1}$ (Lee et al. 2007, Bothwell et al. 2009).
The dispersion in gas fractions does not show
a similar increase (Bothwell et al. 2009), so this suggests
that most of the increase in dispersion in SSFRs reflects
an increased short-term fluctuation of integrated SFRs in 
low-mass galaxies.  Lee et al. (2009) analyzed the statistics
of the SFRs in more depth and confirmed a larger fraction of
stars formed in bursts in low-mass galaxies ($\sim$25\%),
but these still represent only a small fraction of the total
stars formed-- even in the dwarfs the majority of stars 
appear to form in extended events of duration longer than
$\sim$10 Myr.

The most direct way to attack this problem is with deep
color-magnitude diagrams which in principle can provide
age-resolved SFR maps of the galaxies (\S3.X).  As but
one recent example of many studies in this area, Weisz
et al. (2008) used deep HST imaging to derive SFR histories
for 9 dwarf galaxies in the M81 group.  The data reveal
evidence for spatially-localized star formation bursts
over the past 300 Myr (where the technique is sensitive),
with evidence for relatively continuous star formation
over the galaxies.  Further studies of this kind should
be able to provide firmer constraints on the frequency,
durations, and duty cycles of star formation events and
bursts in these low-mass galaxies.



==> localintro.tex <==
%localintro.tex
%updated 032011 NJE
%070811 NJE
%070911 NJE
%051412 NJE minor updates, use ion

\subsection{Historical Perspective and References}\label{localintro}

Star formation in our galaxy has been studied for many years, producing a rich
observational phenomenology and vibrant theoretical discussion. Our focus will
be on those top-level lessons learned from studies of local star formation that
may illuminate studies of other galaxies. For those interested in more detail,
we provide the following brief historical note, with references to useful reviews 
and a few seminal papers.

\citet{2009arXiv0912.1001E} has reviewed the history of star formation studies from the
basic realization that stars must be currently forming, as advocated by Ambartsumian
and Blaauw, through the discovery of the \hi\ hyperfine transition, highlighting
the contributions of Spitzer. 
The problem with the atomic gas was its diffuse nature,
leading to a Jeans mass much larger than stellar masses. The resolution of this
problem came with the discovery of interstellar molecules 
(e.g., \citealt{1968PhRvL..21.1701C,1969Natur.221..626C}), 
%Cheung et al. ammonia, water
especially carbon monoxide (CO) \citep{1970ApJ...161L..43W}, 
which allowed large scale maps of the molecular gas in the Milky
Way (e.g., \citealt{1975ApJ...199L.105S,1986ApJS...60..695C,1988ApJ...327..139C}). 
These showed a very large mass of molecular gas, mostly in large clouds
with masses much in excess of the Jeans mass. Indeed the molecular clouds
presented a problem opposite to that presented by the \hi: 
if collapsing at free-fall, they would vastly
overproduce young stars \citep{1974ARA&A..12..279Z}, an 
issue that has yet to be fully resolved.

Meanwhile, on the theoretical side, \citet{1969MNRAS.145..271L}
%Larson 1969
performed very influential calculations of the evolution of 
a collapsing cloud of initially uniform density.
The modern paradigm (often called the standard model) was laid out
in a review by \citet{1987ARA&A..25...23S},
%Shu, Adams, and Lizano 1987
building on a study by \citet{1977ApJ...214..488S}
%Shu 
of the collapse of a singular isothermal sphere. 
This initial condition (isothermal, with density
$n(r) \propto r^{-2}$) produces a slower and qualitatively different collapse
than do the initial conditions of \citet{1969MNRAS.145..271L}. 
More recent theoretical work has favored a more
dynamical process, in which turbulence and colliding flows play a major role
(e.g., \citealt{2004RvMP...76..125M, 2007ARA&A..45..565M}).
%(Klessen RMPh review and McKee-Ostriker review).
However, observations of low-mass stars suggest infall rates closer
to the Shu solution 
(\citealt{2000prpl.conf..217M,1992ApJ...394..204Z, 1993ApJ...404..232Z}),
% Myers, Evans, Ohashi, Zhou 1992 models, B335 paper) 
or even slower \citep{2010ApJ...710..470D}.
%Dunham et al. 2010 check that this is a reasonable ref for this point

Star formation studies involve a huge range of physical scales (from 100 pc
molecular clouds or complexes to the interiors of stars) and consequently
physical and chemical conditions. In rough evolutionary order, we mention
some reviews for further information. The \hi\ distribution in the Milky Way 
was reviewed by \citet{2009ARA&A..47...27K}
%Kalberla and Kerp  2009
and the molecular gas distribution has been described by
\citet{2001ApJ...547..792D} 
% Dame, Hartmann, and Thaddeus
and \citet{2006PASJ...58..847N}.
%Nakanishi and Sofue
The properties of gas and dust in star
forming regions were reviewed by \citet{1999ARA&A..37..311E},
%Evans99 
with further focus on the cold gas 
by \citet{2007ARA&A..45..339B}.
%Bergin and Tafalla. 
The chemistry of this gas, which plays an integral role in its evolution, 
was reviewed by \citet{1998ARA&A..36..317V},
%vanDishoeck and Blake, 1998
and, in part, more recently by \citet{2009ARA&A..47..427H}.
%Herbst and van Dishoeck, 2009
The nature of interstellar dust was reviewed by \citet{2003ARA&A..41..241D}
%Draine 
and the silicate component by \citet{2010ARA&A..48...21H}.
%Henning.

Turbulence was reviewed by \citet{2004ARA&A..42..211E} and 
\citet{2004ARA&A..42..275S}.
%Elmegreen and Scalo and vice versa 
Magnetic fields were reviewed by \citet{2005LNP...664..137H}
%Heiles and Crutcher (2005, in Cosmic Magnetic Fields,
and their role in star formation summarized by \citet{2010ApJ...725..466C}.
%Crutcher et al. 2010 ApJ
The star formation process has been reviewed many times, but the reviews 
by \citet{1987ARA&A..25...23S} and \citet{2007ARA&A..45..565M}
%Shu87 and McKee-Ostriker07 
are the most influential. A fundamental part of the
star formation process is the generation of winds, jets, and molecular outflows,
which have been reviewed by \citet{1985ARA&A..23..267L}, 
%Lada 1985
\citet{1992A&ARv...3..257B}, and
%Bachiller 1992
\citet{2007prpl.conf..215B}.
%Bally, Reipurth, and Davis 2007. 
Massive stars produce ionized gas, and the \hii\ regions have been reviewed by 
\citet{1979ARA&A..17..345H}
%Habing and Israel 1979
and by \citet{2002ARA&A..40...27C}.
%Churchwell02
The formation of massive stars was reviewed by 
\citet{2007ARA&A..45..481Z}.
%Zinnecker and Yorke 2007.

Studies of the star formation outcomes include evolutionary tracks of 
pre-main-sequence stars (e.g., \citealt{2000ARA&A..38..337C} 
%Chabrier and Baraffe 2000 
for low mass stars and substellar objects). 
These evolutionary calculations are critical for determining the
ages of stars and clusters. 
For more massive stars, it is essential to include accretion in the
evolutionary calculations \citep{1992ApJ...392..667P}
% Palla and Stahler 1992
and high accretion rates cause accreting stars to evolve up the
main sequence \citep{2007ARA&A..45..481Z}.
%Zinnecker and Yorke 
It also seems that accretion and assumptions about initial conditions
may have substantial consequences for the usual methods of determining
ages of young stars (\citealt{2009ApJ...702L..27B, 2010A&A...521A..44B, 
2011ApJ...738..140H}).
% Baraffe et al. and Baraffe and Chabrier on Lithium.
%Hosokawa et al. 2011

There is a major effort to understand the properties and evolution of the 
circumstellar disks because of their role in planet formation, 
with recent reviews by \citet{2010ARA&A..48..205D}
%Dullemond and Monnier 2010
and by Williams \& Cieza (2011, ARA\&A, in press).
Observations indicate that any given stellar system has a roughly 50\%
chance of being a multiple system (\citealt{1991A&A...248..485D,
%Duquennoy and Mayor 1991
2007prpl.conf..133G}).
%Goodwin et al. 2007 in PPV
Theoretical ideas for the formation of multiple star systems are reviewed by
\citet{2007prpl.conf..133G} and \citet{2002ARA&A..40..349T}.
%Tohline, 2002
Observations of stellar clusters in the embedded stage were reviewed by 
\citet{2003ARA&A..41...57L},
% Lada and Lada, 
while more revealed clusters were reviewed by \citet{2010ARA&A..48..431P}.
%Portegies Zwart et al.


==> sfltheory.tex <==
%sfltheory.tex
% formerly known as synthesistheory.tex
%060911
%061511
%070111 new effort after Ringberg
%070811 NJE some cleanup
%080911 NJE
%081111 NJE moved from synthesis to new section on SF relations
%090611 NJE some rearranging and editing

\subsection{Theoretical Ideas for Star Formation Relations}\label{sfltheory}

We describe {\it very} briefly some simple theoretical ideas for
explaining the star formation rate and thresholds. They have
been discussed at greater length by
\citet{2007ARA&A..45..565M} and \citet{2011arXiv1101.3108E},
%Ostriker and McKee ARAA, Elmegreen (2011) 
and, from an observer's perspective, by \citet{2008AJ....136.2782L}.
%Leroy et al. (2008).

Theoretical ideas for explaining the star formation rate can
be crudely divided into two main categories. In the first category,
star formation is determined  at the molecular cloud level.
In one version, midplane pressure 
(\citealt{1989ApJ...338..178E, 1994ApJ...435L.121E})
%(Elmegreen 1989, Elmegreen and Parravano 1994) 
determines the molecular fraction.
In another version, the formation of molecular clouds is primarily
dependent on formation and destruction of \hh, and
not strongly coupled to large scale processes; the star formation
rate is set by the free-fall time of the molecular cloud 
(e.g., \citealt{2005ApJ...630..250K}).
%(e.g., Krumholz and McKee 2005). 

In the other large category, a variety of large scale effects control star
formation. One approach is to turn a fixed fraction of gas into stars every
orbital period, so that $\Sigma(SFR) \propto \Sigma(gas) \Omega$
\citep{1997ApJ...481..703S}.
Disk instability models include free-fall of a section of disk
of fixed height, so that $\rho(SF) \propto \rho/\tff \propto \rho^{1.5}$,
where $\rho \sim \Sigma(gas)/h$, where $h$ is the scale height
(\citealt{1959ApJ...129..243S,1989ApJ...344..685K}).
%(Schmidt 1959, Kennicutt 1989). Can add one with varying scale height.
One simple idea for predicting the star formation rate is that the
{\it volume} SFR density is proportional to the volume density of
gas divided by the free-fall time, $t_{ff} \propto n^{-0.5}$, so that
$\rho(SFR) \propto n/t_{ff} \propto n^{1.5}$. If this local Schmidt law
can be propagated up to galactic scales and converted into surface
density, it nicely explains the slope of the KS relation.
(find the right refs for this)
However, the ISM medium has extreme variations in density and star formation
is strongly concentrated to dense gas. It is not clear that such large
scale averaging of a non-linear function makes sense.
Observations provide no evidence for such a relation on the
scale of  cluster-forming clumps \citep{2010ApJS..188..313W},
%(Wu et al. 2010).
nor on galaxy-wide scales in resolved studies of nearby galaxies
\citep{2008AJ....136.2782L}.
%Leroy et al. (2008) 

There are also several ideas for explaining a threshold in star formation.
The question of whether sharp thresholds exist is discussed elsewhere.
Explanations for thresholds involve large-scale properties.
A gas disk can become unstable to large-scale gravitational instabilities
if $\Sigma(gas) > \alpha_Q{\sigma_g \kappa}/({\pi G})$ 
(Toomre 1964, Martin and Kennicutt 2001). 
This can be modified to account for the stellar potential.
An alternative dynamical criterion involves the shear; instabiliity
requires $\Sigma(gas) > \alpha_A{\sigma_g A}/({\pi G})$.
Parallel to the pressure-mediated view of the SFR, the ability of
phase transitions in atomic gas to form the CNM (Schaye 2004), 
may set a threshold that translates to about 3-10 \msunpc.

As on the scale of molecular clouds (\S \ref{sftheory}), efficiency
is an issue on larger scales. Simulations of galaxy formation tend
to produce runaway star formation, which must be controlled either
by ad hoc assumptions of low efficiency or by invoking negative feedback.
Forming stars can change the phase structure
and pressure (Ostriker latest?) and remove gas from the midplane
(Murray talk at Ringberg, need ref), producing a self-regulating system.
For more intense starbursts, such as those found in mergers, negative
feedback from an AGN is invoked. While these are all plausible, mechanical
feedback from molecular outflows, radiation pressure, HII regions,
and supernovae can also produce positive feedback, at least locally.
Models that rely on feedback from massive stars do not explain why
star formation efficiency is similar in clouds forming only low mass
stars, where such feedback is absent.



==> synthesis.tex <==
%synthesis.tex
%081111 NJE was synthesis_rob.tex

\subsection{Clues from Observations}\label{cluesobs}

Before we embark on an interpretation of the observed
star formation law it is useful to collect the main
conclusions which can be drawn from the observations
of star formation both outside and inside the Galaxy.

On the galactic scale (>1 kpc) we can identify two
distinct star formation regimes.  In the lowest-density
regime star formation is highly dispersed, with young
clusters and HII regions only observed in regions of
unusually high (at that radius) cold gas densities.
This commonly is referred to
as the sub-threshold regime, and although it is most
readily observed in the outer disks of spiral galaxies
it also is found in the interarm regions of some spiral
galaxies and throught the disks of some gas-poor galaxies.
The threshold separating this the low and intermediate-
density regimes is typically of order $\sim$10\,\msun\,pc$^{2}$
or N(H) $\sim 10^{21}$\,cm$^{-2}$, but it may vary systematically.

The cold gas in these regions is predominantly atomic,
though local concentrations of molecular gas are often
found coincident with the sites of star formation.
Compared to the intermediate-density regime which we
next describe the global efficiency of star formation,
which we define as the total SFR per unit gas mass
(or alternatively the ratio of SFR surface density
to gas surface density) is very low, sometimes by
orders of magnitude.   There is no well-defined
Schmidt law in this regime.  [There may be when
you only plot H2 -- but prefer not to complicate the
discussion at this point.]  Plots of SFR surface
density vs gas surface density follow a steep, nearly
vertical relation, but this mainly reflects lack of 
correlation over a region where the SFR has a much
larger dynamic range than the local gas density;
any apparent correlation in the relation is not physical.

At higher densities both the form of the star formation
law and the phase balance of the ISM change dramatically.
In the intermediate density regime ($\sim$10 < $\Sigma_H$ < 200 
\msun\,pc$^{-2}$) star formation tends to be pervasive.
The phase of the cold gas tends to be predominantly (but
not always) molecular.  The SFR surface density is strongly
and tightly correlated with the cold gas surface density, whether expressed
in terms of the total (atomic plus molecular) or only the
molecular surface density.  The characteristic efficiency
or consumption time for the molecular gas is relatively
constant, of order 5--10\%\ per 100 Myr or 100\%\ per 1--2 Gyr.
There is considerable disagreement in the literature about
whether this efficiency is independent of density in
this regime, but the average numbers hold in any case.
The intermediate regime applies within the main optical
radii (R$_{25}$) of most gas-rich, late-type spirals,
many gas-rich irregular galaxies, and the circumnuclear
environments of some less gas-rich spirals.

Unfortunately the limited spatial resolution of extragalactic
molecular line observations (until ALMA at least) make it
impossible to probe for any higher-density star formation
regime, but detailed observations of molecular cloud complexes
in the Milky Way reveal such a regime.  Within molecular
the star formation is observed to be highly localized, with
only a very small (5--10%?) of the gas hosting young
stars, YSOs, and pre-stellar cores.  These latter regions
appear at a threshold surface density of $\sim$200\,\msun\,pc$^{-2}$.
There is no evidence that this threshold density varies
systematically within the Galaxy or elsewhere.
Below this density star formation is absent, and above it
evidences for ongoing star formation are nearly ubiquitous.
Within these dense clumps the effective efficiency of star
formation is very high, of order 50\%; the relatively
low global efficiencies within GMCs is largely a reflection
of the low mass fraction in these dense clumps.  As best
as can be tested this high SFE in clumps also is constant,
independent of the mass of the cloud or the surface density
of the surrounding molecular medium.  This dense clump
scale is as close as a deterministic environment for star
formation as can be found.  Once you form a dense clump
half of its mass will subsequently turn into young stars.

Although current observations of external galaxies cannot
resolve this dense clump regime it can be probed indirectly
though mapping or single-dish measurements of dense molecular
gas tracer species such as HCN.  Observations show evidence
for a linear dependence of total SFR (in mass, not density)
on total HCN mass, extending from Galactic star-forming regions
to normal galaxies and ultraluminous starbursts.  These
observations are consistent with the results above if the HCN
traces the mass in dense molecular clumps.

Finally, in the most extreme starburst galaxy environments
the disk-averaged surface densities of gas (virtually all
molecular) lie in the >200\,\msun\,pc$^{-2}$ regime.
As just mentioned the Schmidt law between SFR and HCN gas
mass remains linear for these galaxies, just as for everything
else.  However the observations require a much higher 
ratio of SFR per unit gas mass (or SFR density/gas density ratio)
by an order of magnitude or more.  The form of the integrated
Schmidt law would suggest that this regime is simply a
non-linear extrapolation of the N = 1.4--1.5 Schmidt law,
but it also could be produced by a vertical shift to a
new (linear) SF mode or a non-linear relation combined with
a linear law in the intermediate regime.

[Sorry I am slipping into interpretation here but that
is anticipating the transition to whereever we take the
text from here.]






==> synthesisobs.tex <==
% synthesisobs.tex
% 060711 NJE
% 060911 NJE
% 070411 NJE
% 070511 NJE
% 070811 NJE
% 072711 NJE
% 080911 NJE

\subsection{Local Tests of Extragalactic Relations} \label{synthesisobs}

There have been few direct tests in our Galaxy of the gas or star 
formation tracers used in extragalactic work, and even fewer of the
inferred star formation laws. Studies of the conversion of CO
observations into column density or mass were discussed in \S \ref{gastracers}.
Here we mention a few tests of relations
between star formation rate and measures of the gas.

Are there tests of \halpha\ versus star counts in HII region/clusters
in the MW or nearby galaxies?
[check new paper by Chomiuk and Povich]
[this part may already be covered in Section 5, so can replace with
reference back to that]

[This can be shortened by reference back to Section 5]
Extragalactic studies have found two kinds of basic star formation ``laws" 
that relate star formation rate to amount of gas.
The first relates SFR to total gas or to gas in some molecular form.
The most well known of these
is a relation between star formation rate surface
density and total gas surface density, as measured by HI and CO, or by CO
alone (Kennicutt98, newest version, Bigiel..). 
Another relation of this kind is one between
far-infrared luminosity and the line luminosity of HCN \jj10, which
is seen in starburst galaxies. 
(Gao and Solomon...)
Since HCN \jj10\ traces much denser
gas than does CO, this is a ``dense gas" relation.

Did GS or anyone ever convert their relation to one for surface densities?
We did only for the dense clumps, not the galaxies.

A second kind of relation is one between star formation rate and
gas divided by a dynamical time, such as:
\begin{equation}
\sigmasfr = \epsilon_{dyn} \sigmagas/\tdyn,
\label{dynamicalrelation}
\end{equation}
where $\epsilon_{dyn}$ is the efficiency of conversion to stars per
dynamical time, \tdyn.

[This can be related to the Krumholz and Tan claim of constant
SFR per free-fall time and I can register my caveats, but I am 
interested to try a more relevant thing, which is a crossing time.]

Check on tests on scale of clouds. Need total SFR and total Gas for MW.

The \lfir-\lhcn\ relation extends to dense clumps in the MW (Wu et al.
2005), as long as $\lfir > \eten{4.5}$ \lsun. If \lfir\ measures
SFR in individual dense clumps, this extension suggests that the
fundamental unit of massive star formation is a dense clump,
suggested by Wu et al. (2005). One problem is that \lfir\ is likely
to underestimate SFR in young clusters (Krumholz and Thompson 2007,
Urban et al. 2010, Gutermuth et al. 2011), perhaps by factors of 3 to 30.
Various authors (Narayanan, Juneau, ...) have pointed out that lines
like those of HCN \jj10\ are not thermalized at lower densities, so
will result in a linear relation even if the underlying relation is
a local version of a non-linear KS law that extends to much lower densities.
It is of course true that the dense gas tracers, by definition, do not
trace all the gas. They do however trace the gas that, in the Milky Way,
is directly involved in star formation (\S \ref{gastracers}).

Using the YSO star counting method to get \sfr\ and extinction maps
to get mean mass surface density of individual, nearby clouds, 
Evans et al. (2009) found that the local clouds all lay well above
the Kennicutt relation. Taken in aggregate, using the mean $\Sigma$(gas),
they lay a factor of 20 above the K98 relation and even farther above
the Bigiel relation. The local clouds were closer to agreement with
the dense gas relation.

Interestingly, the dense gas relation also describes the star formation
rate surface density in starbursts, ULIRGS, and gas-rich QSOs, if the
starburst conversion from CO to mass is used (Daddi et al. 2010).
Both Daddi et al. and Genzel et al. (2010) find that such galaxies
form a separate sequence from normal, but gas-rich, spirals at high z.
(assume that this has been discussed in Rob's sections)

This issue was pursued further by Heiderman et al. (2010), who studied the
$\Sigma$(SFR) on smaller scales using contours of extinction. They limited
the YSOs to Class I objects to ensure that they were still closely related
to their surrounding gas. They found a steep increase in $\Sigma$(SFR)
with increasing $\Sigma$(gas) up to about 130 \msunpc, above which
a turnover was suggested. By adding the dense clumps data from Wu et al.
(2010), they identified a turnover at 129 \msunpc, where the
$\Sigma$(SFR) began to match the dense gas relation found by Wu et al.
(2005). The turnover may be compromised by adding data using a totally
different method, but Lada et al. (2010) found evidence of a very 
similar threshold using completely different arguments.
Gutermuth on the other hand, find a continuation of the steep
slope to higher surface densities in a study including embedded clusters.
They argue for $\Sigma$(SFR) $\propto \Sigma^2$(gas) up to several 100
\msunpc. The differences have to do with details of methodologies, but
all the local studies agree that $\Sigma$(SFR) is strongly localized
to dense gas and much
higher at surface densities above about 100 \msunpc\ 
than predicted by K98 or Bigiel.

A different analysis found that clouds forming stars with masses
over 10 \msun\ satisfied the following relation:
$m(r) \ge 870 \msun (r/pc)^{1.33}$
(\citealt{2010ApJ...716..433K, 2010ApJ...723L...7K}),
where $m(r)$ is the enclosed mass as a function of radius.
This is essentially a criterion they call ``compactness" or it
can be thought of as requiring a central condensation, with
$\rho(r) \propto r^p$, with $p \ge 1.67$.

Dunham (submitted) has compared a subset of clumps in the BGPS catalog
with kinematic distances to the Heiderman-Lada (HL) criterion
for efficient star formation and to the Kauffman-Pillai (KP)
criterion for massive star formation. About half the clumps
satisfy both criteria. Interestingly, \citet{2011ApJ...731...90D}
%Dunham, Robitaille et al.
found that about half the BGPS sample contained at least one
mid-infrared source from the GLIMPSE survey. For the clumps
most securely identified with star formation, 70\% to 80\%
satisfy the HL or KP criteria.

How can we reconcile the extragalactic and MW studies?

Heiderman et al. considered and rejected the most obvious answers,
such as different tracers of gas and star formation, but more work
is needed to firm these arguments up.
They suggested that the difference is a result of resolution.
[refer back to Rob's section on resolved studies.]
Even the best resolution data on other galaxies (excluding the LMC, SMC)
averages over scales of a few 100 pc. For galaxies like the Milky Way,
many clouds will lie within the beam, so $\Sigma$(gas) is highly diluted
compared to a single cloud. Further, in the Milky Way, star formation
is highly localized to the densest gas. If that applies to other galaxies,
the actual star formation occurs only in small regions with $\Sigma$(gas)
far above the mean value that is measured by CO. Further, the use of
\halpha\ as a tracer favors large HII regions that have destroyed their
clouds and expanded. So, improving resolution will probably lead to
more scatter and even an anticorrelation on the smallest scales between
SFR and gas. Indeed, this effect has been seen in studies of 
star formation in nearby galaxies that reach sub-kpc scales (list
some). 
In particular, Liu et al. have quantified the increase in scatter in 
a detailed study of M51. They also find a steepening of the slope of the
KS relation to about 2 at a scale of 200 pc. While this is intriguingly
similar to that found by Gutermuth et al on pc scales, extrapolation of
the fits in Liu to the scales studied by Gutermuth 
would produce much higher slopes. More to the point is that even the
highest $\Sigma$(SFR) seen by Liu et al. at their highest resolution 
lie well below the cloud averaged values in MW clouds. To begin
to match scales, we need at least an order of magnitude better
resolution in nearby galaxies and more large-scale studies of
clouds in the MW, so that we can meet at some resolution.

Consider the following thought experiment. Astronomers in M51
observe the Milky way with 100 pc resolution. In the pixel
centered on the Sun, they would observe no molecular gas and no star
formation indicators. If they degraded their resolution to 300 pc,
they would pick up all the GB clouds, but no localized \halpha\
emission. Assuming they had a super-ALMA, they would measure
$\sigmagas = 0.7$ \msunpc, but they would miss $\sigmasfr = 1.1\ee{-2}$
\sfrkpc.  
With a slightly larger resolution of 500 pc, they would pick up Orion,
with its O stars. They would measure $\sigmagas = 0.4$ \msunpc.
Assuming the relation between \halpha\ luminosity and star formation rate
in K98, they would derive $\sigmasfr = 3\ee{-4}$ \sfrkpc, 
whereas the true value is 8\ee{-3} \sfrkpc. 
This underestimate happens because Orion is not fully sampling the IMF up
to the mass assumed in the K98 relation.
[But earlier, said that Orion makes stars up to 50 Msun. Check this NJE]
If they used the relations for LIR, they would get $\sigmasfr = 1\ee{-4}$
\sfrkpc, low by a factor of 80. 
They would miss almost all the local star formation.
hm, wonder if we know how much diffuse \halpha\
there is around here...
Can I do this for any place in the MW ring?


In some sense, both K98 and Bigiel rely on the fact that
some fraction of the gas within their beams is dense enough to form stars,
or was at some time in the past, and that the fraction $f_{dense}$ increases
with the total amount of gas in the beam. For Bigiel, the relation
between $f_{dense}$ and $\Sigma$(gas) is linear; for K98, 
$f_{dense} \propto \Sigma$(gas)$^{0.4}$.

What happens as we move up the relation to higher values of $\Sigma$(gas)?
Since the emission of CO from a single cloud saturates, values of
$\Sigma$(gas) much greater than 100 really correspond to filling in 
velocity space with more clouds and thus more dense gas. With the K98
relation, and the ansatz that $f_{dense} \propto \Sigma$(gas)
to some power $> 1$,
one eventually reaches a point where all the gas is dense and
rapidly forming stars. This corresponds to the starburst sequence
of Daddi et al. (2010) and Genzel et al. (2010).
Some of the most extreme starbursts can be modeled as a collection
of the kind of dense clumps that form clusters in our Galaxy (Wu et al.
2009). Interestingly, the dense gas and total gas relations of K98
meet at that point.
(assumes Rob has already made the point that Bigiel et al. type relations
cannot explain starbursts)

What are the implications of such a picture? The K98 relation provides
a fine guide to star formation rates on large scales because the fraction
of dense gas is on average related to the mean surface density. But it
should not be taken to apply on the scales where stars actually form,
as many modelers tend to do. Models with resolution that allows
star formation to start at $\Sigma$(gas)$\sim 130$ \msunpc\ 
(re Lada et al. 2010, Heiderman et al. 2010) or that take a very steep
relation between SFR and gas (re Gutermuth et al. 2011) should
be able to reproduce the Bigiel or K98 relations on larger scales.
They may also be able to explain the scatter in the relation and to
study how differences in metallicity and other galactic properties
affect the evolution of galaxies.


==> synthesisques.tex <==

% synthesisques.tex
%061411 [RCK]

\subsection{Key Questions}\label{questions}

The conversion of intergalactic gas into stars requires a series of
transitions in location, density, and, perhaps, chemical state.
Material flows into galaxies and cools to form neutral hydrogen.
Some of that HI becomes dense enough to form a cool neutral phase
(CNM), and (at least in the MW) 
atomic cloud formation is often accompanied by a transition to
predominately molecular gas within sufficiently shielded regions. 
Operating in parallel with these phase transitions is a gradual
transition from gravitationally unbound to bound gas.  In the
ultimate stages of this process sub-regions in molecular clouds become
bound, dense clumps which subsequently evolve into star clusters or
single stars.

Current observations provide clear evidence for the roles of
the largest-scale and smallest-scale components of this chain
of physical processes.  The roles of large-scale dynamical disturbances
such as galaxy-galaxy mergers, bars, and spiral structure in triggering
localized star formation are seen plainly in any atlas of galaxies.
The very existence of the starburst phenomenon testifies to the
non-linear response of the ISM to gas compression on large scales.
Likewise observations of star formation in the MW are providing
increasingly evidence for strong and deterministic coupling between
the molecular gas clumps and cores and the stars which form from
the subcondensations.  

Observations to date, however, do not yet provide a clear
picture of the respective roles of the intermediate-scale
processes in this chain:  the formation of a cool atomic
phase, the formation of molecular gas, and the formation of
bound clouds and/or clumps.  Clearly all are necessary conditions
for star formation, but the processes are physically coupled to
some degree, and could it be that only one (for example the
formation of molecular gas) is sufficient to trigger the others
and determine the SFR by itself?   If such a single 
``critical path" exists, is the critical process the same one
in all galaxies and at all cosmic epochs?

Recasting the observations in the framework of the star
formation law raises another set of often related questions.
When measured in terms of the dependence of the SFR density
on total (atomic plus molecular) gas surface density the 
observed law is characterized by three parameters which
ought to be predictable by theory:  (1) An absolute zeropoint or
global ``efficiency" of star formation which appears to 
be remarkably constant at a given surface density, over a wide
range of parent galaxy and ISM environments; (2) A high-density
slope which may change with surface density;
and (3) A turnover or threshold at low density, which again may
vary systematically within and between galaxies.  Among the
key questions are:  What physical processes set the global 
conversion efficiency of gas into stars, the slope of the 
Schmidt law and the threshold densities?  What are the
separate roles of the atomic and molecular gas components
in determining the observed features in the star formation
law?  Most fundamentally, is the law ultimately shaped by physical
conditions on the galactic scale, as might be suggested by
the nearly universal form of the globally-averaged law (Figure X),
or could it merely be a large-scale artifact of local universal
processes which operate at the sub-cloud level?

Over the past several years these questions have attracted
a flurry of observational, analytical, and numerical studies.
In our view a definitive physical picture has yet to emerge,
and achieving a ``synthesis" at this time lies well beyond
the reach of this review.  Instead we review here the main
ideas which have emerged from observational and theoretical
studies; together they offer important clues to the physics of
large-scale star formation and illuminate some key observations 
and experiments needed in the coming decade.  Our perspective,
unapologetically, is that of observers; for a theoretical
perspective on many of the same issues we heartily recommend
the review by McKee \& Ostriker (2007).




%Are any of these transitions sufficient to ensure star formation?
%In the MW, the formation of dense clumps
%(e.g., those with $\Sigma$(gas)$> 120$ \msun) or prestellar
%cores is nearly sufficient to ensure cluster (star) formation.
%Those with currently low rates of star formation show evidence
%of youth, so barring disruption, they are likely to form stars.
%The formation of large molecular clouds almost always leads to some
%star formation in the MW, but clouds with little gas above $\Sigma$(gas)
%about 120 \msunpc\ can have very little star formation (Lada et al. 2010),
%so molecular cloud formation is not strictly sufficient.
%And certainly most gas currently in molecular clouds does not form stars.
%Surface densities of HI in other galaxies often saturate around 10 \msunyr,
%above which gas is likely to become molecular. Whether the molecular
%(\hh) gas is well traced by the emission from CO depends on metallicity.
%(Rob, are there metal-rich galaxies with lots of HI, but no CO?)
%(Also, I punt on the issue of IGM gas cooling to HI)
%
%Are all of these transitions necessary to allow star formation? 
%Leaving aside the early Universe and atomic cooling halos, 
%molecular gas seems to be required for star formation. Whether the
%molecules themselves are required is controversial. Some argue that
%formation of molecules is the key step (e.g. Gnedin and Kravtsov,
%Krumholz et al. 2009
%and refs therein), but Glover and Clark (2011) have shown that leaving
%out molecular cooling has little effect on the outcome of simulations
%as long as there is a normal amount of dust. They show that [CII]
%emission and dust-gas collisions can cool the gas effectively.
%The point is bit pedantic since normal dust ensures molecules, but
%it is relevant in that the dust is the main arbiter of temperature
%at high densities. Thus we might better say that formation of opaque
%dust clouds, rather than molecular clouds, is the key step.
%Is the formation of a dense clump within a cloud a 
%necessary, as well as sufficient, condition?
%[could discuss Gutermuth here or where it is now..]
%
%What is the role of external influences?
%Compression of molecular gas by molecular outflows, expanding HII regions, 
%wind-driven bubbles, supernovae, and cloud-cloud collisions 
%can trigger star formation
%(e.g., Elmegreen and Lada, ...).
%Such external influences can also disrupt or shred bound gas structures
%(another string of refs)
%Within the MW, the balance sheet for triggering and suppression of
%star formation has never been completely clarified, nor has the global
%significance of triggering (what fraction of star formation in MW
%is stimulated versus spontaneous?).
%On larger scales, galaxy collisions and mergers can either strip gas
%or trigger starbursts.
%[Rob should take over on this one]
%And, of course, dark matter must collect IGM gas in order to make stars...
%
%Is the total SFR of a galaxy controlled by local cloud physics or
%by galaxy-scale processes (or by both)?
%Good place to talk about Toomre instability, shear, ...?
%It seems likely that galaxy scale processes control the
%early steps in the flow of transitions described above, but the
%later ones perhaps only extreme cases, such as mergers.
%
%Do even isolated galaxies experience bursty SF histories?
%There is some evidence in the MW (\S \ref{milkyway}) for this. If so,
%are these the result of positive feedback (triggering) and a limit
%cycle, or are they caused by infall of fresh material?
%
%What similarities and differences show up across the 7 orders of
%magnitude in star formation rates and in star formation rate intensities?

